sGrapp: Butterfly Approximation in Streaming Graphs

We study the fundamental problem of butterfly (i.e. (2,2)-bicliques) counting in bipartite streaming graphs. Similar to triangles in unipartite graphs, enumerating butterflies is crucial in understanding the structure of bipartite graphs. This benefits many applications where studying the cohesion in a graph shaped data is of particular interest. Examples include investigating the structure of computational graphs or input graphs to the algorithms, as well as dynamic phenomena and analytic tasks over complex real graphs. Butterfly counting is computationally expensive, and known techniques do not scale to large graphs; the problem is even harder in streaming graphs. In this paper, following a data-driven methodology, we first conduct an empirical analysis to uncover temporal organizing principles of butterflies in real streaming graphs and then we introduce an approximate adaptive window-based algorithm, sGrapp, for counting butterflies as well as its optimized version sGrapp-x. sGrapp is designed to operate efficiently and effectively over any graph stream with any temporal behavior. Experimental studies of sGrapp and sGrapp-x show superior performance in terms of both accuracy and efficiency.

==> accuracyfigures.tex <==
\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{epinions2.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{mape_ml100k_3.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{MAPE-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{mape-ml10m-2.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{mape-enwiki-2.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{mape-frwiki3.png}}
    
    \caption{[Best viewed in colored.] Accuracy of sGrapp for different values of $\alpha$ and $N_t^W$ }\label{fig:mapes}\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{25semisupervised-mape-epinions.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25semisupervised-mape-ml100k.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25semisupervised-mape-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25semisupervised-mape-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25semisupervised-mape-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25semisupervised-mape-frwiki.png}}
    
    \caption{[Best viewed in colored.] Accuracy of sGrapp-25 for different values of $\alpha$ and $N_t^W$.}
   \label{fig:mapes25}
\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-epinions.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-ml100k.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-mape-frwiki.png}}
    
    \caption{[Best viewed in colored.] Accuracy of sGrapp-50 for different values of $\alpha$ and $N_t^W$ }
   \label{fig:mapes50}
\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-epinions.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-ml100k.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-mape-frwiki.png}}
    
    \caption{[Best viewed in colored.] Accuracy of sGrapp-75 for different values of $\alpha$ and $N_t^W$.}
   \label{fig:mapes75}
\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-epinions.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-ml100k.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ supervised-mape-frwiki.png}}
    
    \caption{[Best viewed in colored.] Accuracy of sGrapp-100 for different values of $\alpha$ and $N_t^W$. }
   \label{fig:mapes100}
\end{figure*}

\begin{figure*}[h]\centering
    \includegraphics[width=\textwidth]{minMAPE.png}
\caption{Minimum approximation MAPE. }
   \label{fig:mapemin}
\end{figure*}

\begin{figure*}[h]\centering
    \includegraphics[width=\textwidth]{maxMAPE.png}
\caption{Maximum approximation MAPE. }
   \label{fig:mapemax}
\end{figure*}

\begin{figure*}[h]\centering
    \includegraphics[width=\textwidth]{probofmapeleq0.15.png}
\caption{Probability of approximation with MAPE less than equal 0.15. }
   \label{fig:mapeprob0.15}
\end{figure*}

\begin{figure*}[h]\centering
    \includegraphics[width=\textwidth]{probofmapeleq0.2.png}
\caption{Probability of approximation with MAPE less than equal 0.2. }
   \label{fig:mapeprob0.2}
\end{figure*}



%\begin{figure*}[h]\centering
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-epinions.png}} 
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-ml100ki.png}} 
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-ml1m.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-ml10mi.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-Enwiki.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/mape/binary/binary-mape-frwiki.png}}
    %\caption{[Best viewed in colored.] MAPE for different sGrapp-binary approximation exponents (x-axes) and adaptive window lengths (y-axes). }\label{fig:mapesbinary}\end{figure*}



\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{epinions.png}} 
    \subfigure{\includegraphics[width=0.3\textwidth]{ml100k.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{frwiki.png}}
   
    \caption{Relative Error of sGrapp over windows for the best obtained MAPE.}\label{fig:realtiveerrors}\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-epinions.png}} \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-ml100k.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 25-err-frwiki.png}}
\caption{Relative Error of sGrapp-25 over windows for the best obtained MAPE.}\label{fig:realtiveerrors25}\end{figure*}

\begin{figure*}[h]\centering
   \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-epinionsi.png}} \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-ml100k.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 50semisupervised-err-frwiki.png}}
 \caption{Relative Error of sGrapp-50 over windows for the best obtained MAPE.}\label{fig:realtiveerrors50}\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-epinions.png}} \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-ml100k.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-enwiki.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ 75semisupervised-err-frwiki.png}}
\caption{Relative Error of sGrapp-75 over windows for the best obtained MAPE.}\label{fig:realtiveerrors75}\end{figure*}

\begin{figure*}[h]\centering
    \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-epinions.png}} \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-ml100k.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-ml1m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-ml10m.png}}
    \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-enwiki.png}}
   \subfigure{\includegraphics[width=0.3\textwidth]{ relativError-optimized-best-frwiki.png}}
 \caption{Relative Error of sGrapp-100 over windows for the best obtained MAPE.}\label{fig:realtiveerrors100}\end{figure*}

%\begin{figure*}[h]\centering
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-epinions.png}} \subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-ml100k.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-ml1m.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-ml10m.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-Enwiki.png}}
    %\subfigure{\includegraphics[width=0.3\textwidth]{figures/optimization/relative_error/binary/binary-err-frwiki.png}}
    %\caption{Relative Error of sGrapp-Binary over windows for the best obtained MAPE. Positive errors are depicted by red upward triangles and negative errors by blue downward triangles.}\label{fig:realtiveerrorsBinary}\end{figure*}

\begin{figure*}[h]\centering
    \includegraphics[width=\textwidth]{mapeComparison.png}
\caption{MAPE of different algorithms.}
   \label{fig:mapecomparison}
\end{figure*}
